Explainable Deepfake Video Detection using Convolutional Neural Network and CapsuleNet

Deepfake technology, derived from deep learning, seamlessly inserts individuals into digital media, irrespective of their actual participation. Its foundation lies in machine learning and Artificial Intelligence (AI). Initially, deepfakes served research, industry, and entertainment. While the concept has existed for decades, recent advancements render deepfakes nearly indistinguishable from reality. Accessibility has soared, empowering even novices to create convincing deepfakes. However, this accessibility raises security concerns.The primary deepfake creation algorithm, GAN (Generative Adversarial Network), employs machine learning to craft realistic images or videos. Our objective is to utilize CNN (Convolutional Neural Network) and CapsuleNet with LSTM to differentiate between deepfake-generated frames and originals. Furthermore, we aim to elucidate our model's decision-making process through Explainable AI, fostering transparent human-AI relationships and offering practical examples for real-life scenarios.

==> chapters/Approval.tex <==
\section*{Approval}
The thesis/project titled "Explainable Deepfake Video Detection
using Convolutional\\ Neural Network and CapsuleNet" submitted
by\\
\begin{enumerate}
\item Gazi Hasin Ishrak (18101503)
\item Zalish Mahmud (18101182)
\item Md. Zami Al Zunaed Farabe (18101394)
\item Tahera Khanom Tinni (17201104)
\end{enumerate}
\\

of Fall 2021 has been accepted by the Department of Computer Science and
Engineering as satisfactory partial fulfillment of the requirements for the degrees of
Bachelor of Science in Computer Science and Engineering or Bachelor of Science in
Computer Science on January 2022.\\
\\
\textbf{Examining Committee:}\\

\vspace{20mm}
\begin{tabular}{p{6cm}p{15cm}}
\begin{tabular}{p{4cm}}

 Supervisor:\\
 (Member)\\
\end{tabular}
&
\begin{tabular}{p{9.5cm}}
\centering

% {\includegraphics[scale=0.15]{images/signature/sign-01narow.png}}\\
\vspace{10mm}
\hline
Dr. Mohammad Zavid Parvez\\
Former Assistant Professor\\
Department of Computer Science and Engineering\\
School of Data and Sciences\\
Brac University \\
\end{tabular}\\
\\ & \\
\begin{tabular}{p{4cm}}
 Co-Supervisor:\\
 (Member)\\
\end{tabular}
&
\begin{tabular}{p{9.5cm}}
\centering

{\includegraphics[scale=0.15]{images/signature/tanzim.png}}\\
\vspace{2mm}
\hline
Md. Tanzim Reza\\
Lecturer\\
Department of Computer Science and Engineering\\
School of Data and Sciences\\
Brac University \\
\end{tabular}\\

\end{tabular}

\newpage

\vspace{30mm}
\begin{tabular}{p{6cm}p{15cm}}

\begin{tabular}{p{4cm}}

 Program Coordinator:\\
 (Member)\\
\end{tabular}
&
\begin{tabular}{p{9.5cm}}
\centering
% {\includegraphics[scale=0.15]{images/signature/sign-01narow.png}}\\
\vspace{12mm}
\hline
Dr. Golam Rabiul Alam\\
Associate Professor\\
Department of Computer Science and Engineering\\
School of Data and Sciences\\
Brac University \\
\end{tabular}\\

\\ & \\

\begin{tabular}{p{4cm}}

Head of Department::\\
(Chair)\\
\end{tabular}
&
\begin{tabular}{p{9.5cm}}
\centering

% {\includegraphics[scale=0.15]{images/signature/sign-01narow.png}}\\
\vspace{12mm}
\hline
Dr. Sadia Hamid Kazi\\
Associate Professor\\
Department of Computer Science and Engineering\\
School of Data and Sciences\\
Brac University \\
\end{tabular}\\

\end{tabular}

\pagebreak

==> chapters/Declaration.tex <==
\section*{Declaration}

It is hereby declared that\\
\begin{enumerate}
\item The thesis submitted is my/our own original work while completing the un-
dergraduate degree at Brac University.
\item The thesis does not contain material previously published or written by a
third party, except where this is appropriately cited through full and accurate
referencing.
\item The thesis does not contain material that has been accepted or submitted for
any other degree or diploma at a university or other institution.
\item We have acknowledged all main sources of help.
\end{enumerate}
\vspace{1cm}\\
\textbf{Student's Full Name & Signature:}\\

\begin{center}
\begin{tabular}{p{9cm}p{9cm}}

\begin{tabular}{p{6cm}}
\centering
{\includegraphics[scale=0.15]{images/signature/sign-01narow.png}}\\
\vspace{2mm}
\hline
Gazi Hasin Ishrak\\
18101503\\ 

\end{tabular}
&
\begin{tabular}{p{6cm}}
\centering
{\includegraphics[scale=0.15]{images/signature/zalish.png}}\\
\vspace{2mm}
\hline
Zalish Mahmud\\
18101182\\
\end{tabular}\\
\\ & \\
\\ & \\
\begin{tabular}{p{6cm}}
\centering
{\includegraphics[scale=0.15]{images/signature/farabe.png}}\\
\vspace{2mm}
\hline
Md. Zami Al Zunaed Farabe\\
18101394\\
\end{tabular}
&
\begin{tabular}{p{6cm}}
\centering
{\includegraphics[scale=0.15]{images/signature/tahera.png}}\\
\vspace{2mm}
\hline
Tahera Khanom Tinni\\
17201104\\
\end{tabular}\\

\end{tabular}
\end{center}
\pagebreak

==> chapters/Dedication.tex <==
\section*{Dedication}
We wholeheartedly dedicate our work to our beloved parents who have always been supporting us throughout our ups and downs with their moral, emotional, and financial support.
Lastly, our work is dedicated to the improvement of deep fake detection techniques that have been securing people’s life and their image.
\pagebreak

==> chapters/futureWork.tex <==
Our model has shown promising results with the given dataset. However, we are looking forward to using different datasets to feed into our model to see how it performs. Moreover, we want to merge multiple datasets and train our model to ensure unbiased deep learning.  We have used DeepFace model to crop the faces from the video frames. However, in our comparison, we have seen that our model has given less accuracy in cropped faces. In the future, we would like to improve the accuracy by changing the frame's properties such as brightness, contrast, and gray scale. Additionally, we would like to work on different frame rates as well. We can change our current frame rate, which is 1 frame per second to 2 or 3 frames per second which will enlarge our dataset and can be beneficial to improve our model’s accuracy. We would also like to work on other meta areas that we have reviewed in various papers such as, audio spoofing, tracking iris and nose pointer locations. As we have implemented explainable Ai, we would like to work on the activation heatmaps and try to find a pattern of our model of detecting fake videos. We look forward to working on these shortcomings and scopes to research further to improve our model.

